Supporting the Careers of Developers with Disabilities: Lessons from Zup Innovation

People with still face discrimination, which creates significant obstacles to accessing higher education, ultimately hindering their access to high-skilled occupations. In this study we present Catalisa, an eight-month training camp (developed by Zup Innovation) that hires and trains people with disabilities as software developers. We interviewed 12 Catalisa participants to better understand their challenges and limitations regarding inclusion and accessibility. We offer four recommendations to improve inclusion and accessibility in Catalisa-like programs, that we hope could motive others to build a more inclusive and equitable workplace that benefits everyone.

==> extra.tex <==

\iffalse

\geraldo{
Quanto aos pontos observados de melhorias:
\begin{itemize}


%\item Uma outra estratégia sugerida para evitar longas interrupções do assunto com dúvidas, é ter um momento para dúvidas durante a aula, após a explicação do assunto; \gnote{acho que ja tem um sobre interrupção. esse tem algo diferente?}   \geraldo{Não vi a outra de interrupção}
\item Passar muito conteúdo teórico de uma vez pode ser prejudicial para o entendimento, dividir a manhã para a teoria e a tarde para práticas pode ser uma boa estratégia; \gnote{nao vi a inclusao?}   \geraldo{Isso ajuda por exemplo no ponto dos leitores de tela e está colando código no chat. O compleicado é ter isso enquanto está se passando um assunto, mas na prática, ajuda eles. Daí criar essa separação permite além do melhor entendimento, segundo eles, práticas e teorias mais acessiveis}
%\item Suporte de professores e mentores em horários alternativos; \gnote{nao sei se é sobre inclusao?}   \geraldo{Aqui também concordo}
\item Passar assunto que será visto um dia antes da aula para que se possa construir dúvidas \gnote{nao sei se é sobre inclusao?}   \geraldo{Aqui quem comentou foi a pessoa que tem déficit de atenção, que ter o assunto antes ajudaria a ter dúvidas para a aula, pq basicamente só conseguia ter duvidas deposi de assitir a gravação em 2x}
%$\item Se possível, usar o terminal para ações de git, montagem de ambiente, dentre outras ações; \gnote{nao vi a inclusao?}   \geraldo{Aqui quem comentou foi Davi e Victor, que algumas coisas eram ensinas no intelij, mas fazer pelo terminal era mais universal e acessivel para todos}
%\item Rodar um NPS ao final da formação para coleta de feedbacks. \gnote{acho que nao é sobre inclusao}   \geraldo{Aqui acho que entraria como uma recomendação geral para a formação, ter essas intervencoes para coletar melhorias para o programa cosntantemente e nao vendermos bala de prata}
\end{itemize}
}

\fi

%\item Sempre que possível detalhar onde está clicando e descrever imagens. Procurar não usar termos como “clique aqui”, “veja isso”, “Arraste isso para lá”;

\iffalse
\subsection*{RQ3: What changes were made in order to make the training camp more inclusive?}

%\begin{itemize}
%\item A empresa fornece acesso a recursos de adaptação para o ambiente de estudo e equipamentos de tecnologia assistiva para viabilizar a participação nas aulas e práticas; \gnote{ja falamos na RQ1}
%\item O programa de treinamento incentiva o trabalho em equipe e a inserção de práticas para a melhoria de soft skills no dia a dia dos estudantes; \gnote{ja falamos na RQ1}
%\item Ter um time de mentores capacitados e preparados para lecionar com práticas de ensino inclusivas, procurando atender cada estudante da melhor forma possível;\gnote{falamos na RQ2}
%\end{itemize}


% \subsubsection*{Accessibility by design}

% \nota{um achado que eu acho muito interessante é que os trabalhos desenvolvidos por eles foram todos accesiveis by design, que é algo que a literatura reporta que o pessoal nao tem costume. Ter pcds no time faz com que o time se preocupe com acessibilidade, o que melhora a qualidade do software no geral (ex., o prof que quase todos reclamaram não ter meios acessiveis, teve que aprender como ser inclusivo).}

% \nota{um trabalho sobre: (Accessibility in Software Practice: A Practitioner’s
% Perspective) https://arxiv.org/pdf/2103.08778.pdf}\gnote{rola cita-lo ali na sec 2?}



\geraldo{
Quanto às boas práticas de inclusão percebidas durante o programa de formação:

\begin{itemize}
%\item O ambiente de estudo proporciona desafios reais, cobranças e busca por resultados e melhorias durante a formação; \gnote{nao acho que esse seja de inclusao} \geraldo{Gustavo, nesse ponto, Katia, Davi e Victor que já tinham experiências anteriores destacaram que a existência de desafios reais e cobranças os ajudaram a se sentir incluídos e responsáveis por aquilo que estavam fazendo. Katia comentou que em uma empresa anterior praticamente foi contratada para fazer nada. Eles comentam sobre não se sentirem como "cota" e sim terem responsabildiades e serem cobrados como todos } \gnote{escrevi na RQ2}
\item Planejar toda a condução da formação com antecedência, procurando projetar um storytelling entre os conteúdos, aulas e práticas que serão passadas foi um ponto de destaque. Isso possibilita que os estudantes se antecipem aos assuntos que serão vistos e a unirem os conteúdos aprendidos no desenvolvimento dos desafios e projetos; \gnote{nao acho que seja sobre inclusao} \geraldo{Isso foi outro ponto de destacado como alguns como ponto estratégico da formação. O fato de planejar com antecedência permite observar momentos exatos onde será preciso alguma intervenção ou mais atenção com a acessibildiade. Eles disseram que sentiram um cuidado nisso durante o Catalisa.}
% 
\item Ao final da formação de 5 meses, a inserção em projetos reais da empresa por 3 meses, ainda durante a formação, possibilita o contato dos estudantes de forma antecipada com o cotidiano de squads de desenvolvimento. \gnote{nao acho que seja sobre inclusao} \geraldo{esse ponto vai na linha do trabalho em grupo. Antes do Catalisa alguns comentaram sobre chegarem com o sentimento de trabalho individual e de não conseguirem trabalhar com outras pessoas. Durante aprendem o trabalho em grupo. O Davi comentou que a experiência que ele está tendo no Itaú consolida o sentimento de que ele está preparado para trabalhar em times com pessoas com e sem deficiência.}
% 
%\item Exercícios e desafios com entregas mínima, média e máxima possibilitavam a entrega de quem tinha dificuldades, gerando satisfação, e o indicativo de melhorias a serem construídas; \gnote{nao sei se é sobre inclusao} \geraldo{Esse ponto aqui realmente... mais de uam pessoa comentou que foi muito importante para se sentirem motivados e engajados ao longo da formação, porém, acho que entra mais como um gatilho de satisfação/softskills de ter concluido algo msm não conseguindo mandar tão bem em um assunto}
%\item Feedbacks constantes de professores e mentores eram muito importantes para se ter noção de onde se está e para onde podem ir para continuar melhorando. \gnote{tambem nao sei se é sobre inclusao} \geraldo{Acho que vai na msm linha do de cima}
\nota{os dois tópicos acima (feedback e entregas) eu citaria rapidamente no tópico onde descreve que eles se sentem valorizados, desafiados e tals (são mais que cotas)}
\item Compartilhar códigos desenvolvidos nas práticas em tempo real pelo chat e depois da aula colocar os códigos no Github de forma acessível, montando um readme explicando o projeto e sua execução;
%\item Montar códigos em tempo real durante as aulas, em conjunto com os estudantes, procurando explicar detalhes da implementação; \gnote{explicado na RQ2}
\item Dividir os encontros em momentos teóricos e práticos aparenta ser mais inclusivo, inclusive para quem precisa ouvir o conteúdo que é escrito em tela, possibilitando um chaveamento mais assertivo;
%\item Aulas interrompidas para dúvidas podem gerar dificuldades de compreensão, logo, a disponibilização de vídeos relativos a parte téorica pré-gravados seria importante para evitar essa situação;\gnote{descrito na RQ2}
\item Validar aspectos de acessibilidade em software, IDEs e ferramentas a serem utilizadas na formação com antecedência. Durante a formação, mais uma vez validar com os estudantes a acessibilidade das ferramentas escolhidas;
\end{itemize}
}

\gnote{eu lembro que teve alguem que mencionou que colar o código no chat nao era inclusivo, pois o assistente virtual de leitura lia enquanto o professor falava?}
\geraldo{Isso, foi a Ana que trouxe isso, mas nos momentos de teória + Pratica, num tópicos mais pra baixo comento sobre dividir teoria e prática para tornar isso possivel sem ter a fala do professor por cima}
\nota{o que é inclusivo não é colar na lousa do google meet não?}


\fi
